LVP-CLIP:Revisiting CLIP for Continual Learning with Label Vector Pool

Continual learning aims to update a model so that it can sequentially learn new tasks without forgetting previously acquired knowledge. Recent continual learning approaches often leverage the vision-language model CLIP for its high-dimensional feature space and cross-modality feature matching. Traditional CLIP-based classification methods identify the most similar text label for a test image by comparing their embeddings. However, these methods are sensitive to the quality of text phrases and less effective for classes lacking meaningful text labels. In this work, we rethink CLIP-based continual learning and introduce the concept of Label Vector Pool (LVP). LVP replaces text labels with training images as similarity references, eliminating the need for ideal text descriptions. We present three variations of LVP and evaluate their performance on class and domain incremental learning tasks. Leveraging CLIP's high dimensional feature space, LVP learning algorithms are task-order invariant. The new knowledge does not modify the old knowledge, hence, there is minimum forgetting. Different tasks can be learned independently and in parallel with low computational and memory demands. Experimental results show that proposed LVP-based methods outperform the current state-of-the-art baseline by a significant margin of 40.7%.

==> sec/backup.tex <==
\begin{table*}[]
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{cccccccccccc}
\toprule
Method      & Task 1 & Task 2 & Task 3 & Task 4 & Task 5 & Task 6 & Task 7 & Task 8 & Task 9 & Task 10  \\
\hline
iCaRL~\cite{rebuffi2017icarl}  &88.7 &78.1 &72.4 &67.2 &63.7 &60.2 &56.4 &54.4 &51.9 &49.5 \\
ARI~\cite{wang2022anti} &88.6 &86.9 &85.8 &84.6 &83.1 &81.8 &81.6 &81.0 &80.2 &80.9 \\
CoOp~\cite{zhou2022learning} &95.8 &90.7 &85.2 &83.4 &80.8 &75.8 &74.7 &71.7 &71.3 &67.6  \\
Continual-CLIP~\cite{thengane2022clip}        &96.7 &92.2 &86.0 &80.4 &77.5 &75.8 &73.0 &71.4 &69.8 &66.7 \\
AttriCLIP~\cite{wang2023attriclip}    &97.8 &93.7 &91.0 &87.5 &84.7 &82.5 &82.3 &81.9 &81.7 &81.4\\
\midrule 
\methoda    &96.0 &92.3 &89.2 &88.0 &86.3 &84.6 &82.8 &81.4 &81.2 &80.2\\
\methodb     & 96.4   & \textbf{93.9}   & 90.6   & \textbf{89.2}   & \textbf{87.4}   & \textbf{85.7}   & \textbf{84.2}   & \textbf{82.8} & \textbf{82.8} & \textbf{82.0}\\
\methodc &&&&&&&&&&81.1\\
\midrule  
 Upper-bound &&&&&&&&&&86.5\\ 
\bottomrule
\end{tabular}
}
\caption{CIFAR100~\cite{krizhevsky2009learning}}
\label{tab:cifar100}
\end{table*}

\begin{table*}[]
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{cccccccccccc}
\toprule
Method      & Task 1 & Task 2 & Task 3 & Task 4 & Task 5 & Task 6 & Task 7 & Task 8 & Task 9 & Task 10  \\
\hline
iCaRL~\cite{rebuffi2017icarl}  &82.1 &80.6 &75.5 &70.1 &68.1 &65.8 &62.5 &61.3 &60.7 &59.5 \\
ARI~\cite{wang2022anti} &87.6 &85.4 &83.1 &82.6 &80.4 &80.8 &80.5 &80.1 &79.6 &79.3 \\
CoOp~\cite{zhou2022learning} &89.2 &83.2 &76.7 &79.8 &79.9 &82.34 &79.7 &80.1 &80.3 &79.3  \\
Continual-CLIP~\cite{thengane2022clip} &93.3 &87.6 &83.1 &81.7 &80.5 &80.2 &79.3 &78.5 &76.9 &75.4 \\
AttriCLIP~\cite{wang2023attriclip} &95.4 &89.4 &84.5 &86.7 &84.4 &86.6 &85.9 &85.6 &86.9 &83.3\\
\midrule 
\methoda & 93.6   & 90.0   & 88.8   & 90.7   & 91.8   & 92.8   & 92.4   & 91.9 & 91.5 & 91.8\\
\methodb  & 93.6   & \textbf{91.0}   & \textbf{90.1}   & \textbf{91.5}   & \textbf{92.6}   & \textbf{93.5}   & \textbf{93.1}   & \textbf{92.4} & \textbf{92.2} & \textbf{92.5}\\
\methodc &&&&&&&&&& 92.5\\
\midrule 
Upper-bound &&&&&&&&&& 96.0\\
\bottomrule
\end{tabular}}
\caption{ImageNet100~\cite{deng2009imagenet}}
\label{tab:imagenet100}
\end{table*}


\begin{table*}
  \centering
  %\resizebox{1\linewidth}{!}{
  \begin{tabular}{c c c c | c c c}
    \toprule
     Method & Buffer size & CIFAR100 & ImageNet100 & Method & ModelNet40 & ShapeNet\\
    \midrule
    iCaRL & 0  &49.5 &63.5 & 74.8\\
    ARI & 0 &80.9 & 64.3 &75.5\\
    CoOp & 0 &67.6 &68.3 &78.3\\
    Contimual-CLIP & 0 &66.7 &70.6 &89.1\\
    AttriCLIP & 0 &81.4 &72.3 &83.7\\
    \midrule
    {\methoda} &0 &80.2 &85.5 &87.8\\
    {\methodb} & 0 & 82.0 & - & - \\
    {\methodc} & 0 & 81.5 & - & 89.6 \\
    \midrule
    Upper-bound  & - & 86.5 & & \\
    \bottomrule
  \end{tabular}
  %}
  \caption{Testing accuracy on CIFAR100 of \method. * from L2p}
  \label{tab:domain_incremental}
\end{table*}

\begin{table*}
  \centering
  %\resizebox{1\linewidth}{!}{
  \begin{tabular}{c c c c c}
    \toprule
     Method & Buffer size & DomainNet & OfficeHome & CORe50\\
    \midrule
    EWC & 0  &57.0 &63.5 & 74.8\\
    LwF & 0 &58.4 & 64.3 &75.5\\
    L2P~\cite{wang2022learning} &  0&63.3 &68.3 &78.3\\
    S-iPrompts & 0 &67.8 &70.6 &89.1\\
    DualPrompt~\cite{wang2022dualprompt} & 0 &68.8 &72.3 &83.7\\
    \midrule
    {\methoda} &0 &70.1/72.4* &85.5 &87.8\\
    {\methodb} & 0 & 70.9/74.0* & - & - \\
    {\methodc} & 0 & 68.8/74.0* & - & 89.6 \\
    \midrule
    Upper-bound  & - & 79.1 & & \\
    \bottomrule
  \end{tabular}
  %}
  \caption{Testing accuracy on CIFAR100 of \method. * from L2p}
  \label{tab:domain_incremental}
\end{table*}

\begin{table*}[]
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{cccccccccccc}
\toprule
Method      & Task 1 & Task 2 & Task 3 & Task 4 & Task 5 & Task 6 & Task 7 & Task 8 & Task 9 & Task 10  \\
\hline
BiC~\cite{wu2019large}         & 97.8   & 95.5   & 88.5   & 86.9   & 84.3   & 83.1   & 79.3   & 74.2   & 70.7   & 59.2   \\
RPS-Net~\cite{rajasegaran2019random}     & 97.7   & 94.6   & 90.3   & 88.2   & 86.7   & 82.5   & 78     & 73.6  & 68.4  & 58.3   \\
LUCIR~\cite{hou2019learning}+DDE~\cite{hu2021distilling}   & 97.9   & 96.1   & 91.4   & 88.9   & 87.5   & 84.6   & 80.4   & 75.1  & 71.4  & 59.8   \\
LUCIR~\cite{hou2019learning}+GeoDL~\cite{simon2021learning} & 97.8   & 96.5   & 92.2   & 90.3   & 88.4   & 85.8   & 81.3   & 76.3  & 72.2 & 60.3    \\
I3DOL~\cite{dong2021i3dol}       & 98.1   & 97     & 93.4   & 91.1   & 89.7   & 88.2   & 83.5   & 77.8  & 73.1  & 61.5   \\
InOR-Net~\cite{dong2023inor}    & 98.1   & 97.5   & 95.6   & 93.7   & 91.4   & 90.3   & 85.9   & 79.2  & 74.6  & 63.9  \\
\midrule
\methoda        & 95.9   & 96.4   & 95.1   & 91.6   & 90.5   & 86.0   & 82.3   & 81.0 & 80.7 & 75.7  \\
\methodb        & 95.9   & 96.6   & 94.9   & 91.6   & 91.1   & 86.1   & 82.6   & \textbf{81.3} & \textbf{81.0} & \textbf{76.0}  \\
\methodc &    &    &    &    &    &    &   &  &  & \textbf{77.9}  \\
\bottomrule
\end{tabular}}
\caption{Accuracy of different continual learning methods on ModelNet40~\cite{wu20153d}. The accuracy of Task $t$, $t \in \{1,2,...,10\}$ reported here is the test accuracy averaged over all the previous tasks.}
\label{tab:modelnet}
\end{table*}

\begin{table*}[]
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{cccccccccccc}
\toprule
Method      & Task 1 & Task 2 & Task 3 & Task 4 & Task 5 & Task 6 & Task 7 & Task 8 & Task 9   \\
\hline
BiC~\cite{wu2019large}         & 97.4   & 92.1   & 86.7   & 81.5   & 76.4   & 73.7   & 69.8   & 67.6   & 64.2      \\
RPS-Net~\cite{rajasegaran2019random}     & 97.6   & 92.5   & 87.4   & 80.1   & 77.4   & 72.3   & 68.4     & 66.5  & 63.5    \\
LUCIR~\cite{hou2019learning}+DDE~\cite{hu2021distilling}   & 97.6   & 93.1   & 88.7   & 82.1   & 78.5   & 74.5   & 71.2   & 67.9  & 64.8    \\
LUCIR~\cite{hou2019learning}+GeoDL~\cite{simon2021learning} & 97.6   & 93.7   & 89.3   & 82.9   & 79.3   & 75.2   & 71.9   & 69.4  & 66.3     \\
I3DOL~\cite{dong2021i3dol}       & 97.5   & 94.4     & 90.2   & 84.3   & 80.5   & 76.1   & 73.5   & 70.8  & 67.3  \\
InOR-Net~\cite{dong2023inor}    & 97.5   & 95.6   & 92.4   & 86.7   & 83.1   & 79.2   & 76.0   & 73.5  & 69.4    \\
\midrule
\methoda        & \textbf{98.9}   & \textbf{98.1}   & \textbf{97.0}   & \textbf{90.3}   & \textbf{82.3}   & \textbf{79.2}   & \textbf{79.9}   & \textbf{76.7} & \textbf{78.2}  \\
% \methodb        & 95.9   & 96.6   & 94.9   & 91.6   & 91.1   & 86.1   & 82.6   & \textbf{81.3} & \textbf{81.0}  \\
\bottomrule
\end{tabular}}
\caption{Accuracy of different continual learning methods on ShapeNet~\cite{chang2015shapenet}. The accuracy of Task $t$, $t \in \{1,2,...,10\}$ reported here is the test accuracy averaged over all the previous tasks.}
\label{tab:shapenet}
\end{table*}


% \begin{table}
%   \centering
%   \resizebox{1\linewidth}{!}{
%   \begin{tabular}{lc c c}
%     \toprule
%      Method & CF100 + IN100 + CR50 + DN & ablation\\
%     \midrule
%     L2P~\cite{L2P} & 37.4 & -\\
%     DualPrompt~\cite{DualPrompt} & 40.3 & 83.1\\
%     \midrule
%     {\methoda} &80.9 & 82.7\\
%     {\methodb} &\bf{81.0} & 83.7\\
%     {\methodc} &79.4 &83.3\\
%     \midrule
%     %DualPrompt-ablation &83.1\\
%     %{\methoda-ablation} &82.9\\
%     %{\methodb-ablation} &83.9\\
%     %{\methodc-ablation} &83.3\\
%     Upper-bound  & 87.1 & 88.9\\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Testing accuracy on CIFAR100 + ImageNet100 + CORe50 + DomainNet. 
%   %The LVP memory is $\mem = (1\times100 + 1\times100 + 8\times50 + 6\times345)\times\ebdim = 13.6 \unit$.
%   }
%   \label{tab:ctil}
% \end{table}

{\bf Adaptive {\labelpool} for DomainNet.*}
DomainNet has 6 domains which are "Clipart", "Infograph", "Painting", "Quickdraw", "Real", "Sketch" and the testing accuracy of (\methoda) for every single domain are 82.9\%, 56.0\%, 76.3\%, 46.1\%, 87.2\%, 73.4\% respectively. The "Quickdraw"(46.1\%) domain is the one that drags the total accuracy. However, this domain is so different from the others that it is even possible to identify it from the others. We design two simple {\labelpool} $L^{Quickdraw}_{yes} = \{\frac{1}{345}\sum^{345}_{i=1} L^{Quickdraw}_{i}\},\poolsize=1$ and $L^{Quickdraw}_{no} = \{\frac{1}{345*5}\sum^{345*5}_{i=1} L^{NotQuickdraw}_{i}\},\poolsize=1$. In short, $L^{Quickdraw}_{yes}$ is the mean of the {\labelpool} of the "Quickdraw" domain and $L^{Quickdraw}_{no}$ is the mean of the {\labelpool} of the other domains. We validate this design on the testing images of all domains and get 99.98\% accuracy in determining the correct ID(Quickdraw or not Quickdraw). We train a classifier over all the training data of "Quickdraw" domain and get 62.5\% accuracy on the testing data. Each time when inference a testing image, it will calculate the similarity with $L^{Quickdraw}_{yes}$ and $L^{Quickdraw}_{no}$ to identify if it is an image in "Quickdraw" domain or not. If it is, the image embedding will forward to the "Quickdraw" classifier and if not, the image just follows the proposed methods we desirable in \cref{sec:4}.


{\bf Why LVP-C is sometimes better, sometimes the same, and sometimes worse compared to LVP-I and LVP-IT?} 
As demonstrated in \cref{sec:4}, the $\theta$ is a TS parameter but optimized on very limited data. The optimization objective of $\theta$ is to distinguish the difference between {\labelpool} of each class and classify them but not classify any training/testing data. The performance of LVP-C relies on 2 points, [1] the quality of LVP in representing the training data, [2] the pattern hiding in the LVP. For the former, the better the quality the better the performance. For the latter, the more the patterns and the more important the pattern, the better performance. For LVP-I and LVP-IT, when calculating the similarities, each element of the vector has the same importance but the LVP-C makes it possible to learn the hidden pattern inside the LVPs to make better resutls.

\section{Extra experiments}

\subsection{Class Incremental on 3D Point Cloud}
To demonstrate the grate adaptability of our proposed methods, we also evaluated our approach on two public point cloud datasets, namely ModelNet40~\cite{wu20153d} and ShapeNet~\cite{chang2015shapenet}.

%{\bf Datasets.} 
%ModelNet40~\cite{wu20153d} contains 12,311 CAD models covering 40 categories, with 9,843 objects in the training set and 2,468 objects in the testing set. 
We split ModelNet40 into 10 tasks with 4 classes in each task. %ShepNet~\cite{chang2015shapenet} contains 45,832 training samples and 6,640 testing samples across 55 classes. 
For ShapeNet, to keep consistent to the previous work~\cite{dong2023inor}, we use 53 of the 55 classes, excluding 'airplane' and 'ashcan'. The dataset is divided into 9 tasks, each containing 6 classes, except for the final task with 5 new classes.

{\bf Baselines.} 
%We compared our method with existing 2D~\cite{wu2019large,rajasegaran2019random,hou2019learning,hu2021distilling,simon2021learning} and 3D~\cite{dong2021i3dol,dong2023inor} class incremental methods, all baseline utilize PointNet~\cite{qi2017pointnet} as feature extractor. BiC~\cite{wu2019large} addresses the correction of bias introduced by new categories within the classifier. RpS-Net~\cite{rajasegaran2019random} aims to optimize information flow for new tasks. LUCIR~\cite{hou2019learning} finds that the weight norm of new classes is significantly larger than old ones, thus it proposes to utilize a cosine classifier to avoid the influence of biased classifiers. DDE~\cite{hu2021distilling} seeks to explore the causal relationship between old and new categories. GeoDL~\cite{simon2021learning} enhances knowledge distillation techniques by measuring the similarity between previous and current responses using geodesic paths. I3DOL~\cite{dong2021i3dol} is a rehearsal-based method, it addresses 3D class-incremental learning by introducing an adaptive-geometric centroid module and a geometric-aware attention module to capture unique 3D geometric and local features, mitigating catastrophic forgetting. Additionally, a score fairness compensation strategy is employed to correct biased predictions for new classes. The extension work~\cite{dong2023inor} introduces a category-guided geometric reasoning module to capture intra-class 3D features and a dual adaptive fairness compensation strategy to adjust both weights and prediction scores, effectively addressing catastrophic forgetting.
We compare our methods with existing SOTA methods for point cloud continual learning, namely five 2D methods BiC~\cite{wu2019large}, RpS-Net~\cite{rajasegaran2019random}, LUCIR~\cite{hou2019learning}, DDE~\cite{hu2021distilling}, GeoDL~\cite{simon2021learning}, and two 3D methods I3DOL~\cite{dong2021i3dol}, InOR-Net~\cite{dong2023inor}, all baseline utilize PointNet~\cite{qi2017pointnet} as feature extractor. 

{\bf Results.} 
%In this section, we conduct experiments on 3D point cloud using the PointCLIPv2~\cite{zhu2023pointclip} framework, which generates CLIP-preferred images through realistic projection, and utilizes GPT-3~\cite{GPT3} to generate text with richer 3D semantics.  We compare the proposed method with the prior arts on ModelNet40~\cite{wu20153d} and ShapeNet~\cite{chang2015shapenet} with the results summarized in Tab.~\ref{tab:3dcls}.
From the results of ModelNet40 in Tab.~\ref{tab:3dcls}, we can see that our method significantly outperforms the second best method by 12.1\%, without requiring rehearsal buffer size. For ShapeNet, our method outperforms all baselines, achieving the best performance. Notably, it surpasses the second best model, InOR-Net~\cite{dong2023inor}, by 8.8\%. For this dataset, we omit the results of {\methodb}\;, since PointCLIPv2~\cite{pointclipV2} does not provide the optimal text prompt. Using basic text prompt, like 'Point Cloud Depth Map of a [Class]', yields a zero-shot result 29.1\%, indicating poor  text quality, which negatively impacts performance. A detailed discussion on text quality can be found in sec.~\ref{sec:ablation}.



\begin{table}
  \centering
  \resizebox{1\linewidth}{!}{
  \begin{tabular}{lc c c c}
    \toprule
     Method & Buffer size & ModelNet40~\cite{wu20153d} & ShapeNet~\cite{chang2015shapenet}\\
    \midrule
    BiC~\cite{wu2019large} &   &59.2* &64.2*\\
    RPS-Net~\cite{rajasegaran2019random} &  &58.3* & 63.5*\\
    LUCIR~\cite{hou2019learning}+DDE~\cite{hu2021distilling} &  &67.6* &64.8*\\
    LUCIR~\cite{hou2019learning}+GeoDL~\cite{simon2021learning} & 800/1000 &60.3* &66.3*\\
    I3DOL~\cite{dong2021i3dol} &  &61.5* &67.3*\\
    InOR-Net~\cite{dong2023inor} &  &63.9* &69.4*\\
    \midrule
    {\methoda} &0 &75.7\phantom{*} &78.2\phantom{*}\\
    {\methodb} & 0 & 76.0\phantom{*} & -\phantom{*}\\
    {\methodc} & 0 & \bf{77.9}\phantom{*} & \bf{83.8}\phantom{*}\\
    \midrule
    Upper-bound  & - & 88.9\phantom{*} & 96.0\phantom{*}\\
    \bottomrule
  \end{tabular}
  }
  \caption{Results on 3D class-incremental learning. Buffer size 800/1000 represents storing 800 and 1000 samples in the exemplar set for ModelNet40 and ShapeNet, respectively. The LVP comlesity is $O=1[\poolsize]\times40[\clsnum]=40$ for ModelNet40 and $O=1[\poolsize]\times53[\clsnum]=53$ for ShapeNet. * is result from InOR-Net~\cite{dong2023inor}.}
  \label{tab:3dcls}
\end{table}
